Learning Emotion from 100 Observations: Unexpected Robustness of Deep Learning under Strong Data Limitations

One of the major downsides of Deep Learning is its supposed need for vast amounts of training data. As such, these techniques appear ill-suited for NLP areas where annotated data is limited, such as less-resourced languages or emotion analysis, with its many nuanced and hard-to-acquire annotation formats. We conduct a questionnaire study indicating that indeed the vast majority of researchers in emotion analysis deems neural models inferior to traditional machine learning when training data is limited. In stark contrast to those survey results, we provide empirical evidence for English, Polish, and Portuguese that commonly used neural architectures can be trained on surprisingly few observations, outperforming $n$-gram based ridge regression on only 100 data points. Our analysis suggests that high-quality, pre-trained word embeddings are a main factor for achieving those results.

==> PEOPLES 2020 - Emotion in small datasets/custom_preamble.tex <==
\usepackage[T1]{fontenc}
\usepackage{mathtools}
\usepackage{multirow}
\usepackage{subcaption}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{booktabs}
\usepackage{rotating}
\usepackage{enumitem}
\usepackage{todonotes}
\usepackage[linewidth=1pt]{mdframed}

\newcommand{\textsuper}[1]{$^\text{#1}$}
\newcommand{\textcomment}[1]{\textcolor{red}{[#1]}}
\newcommand{\textsub}[1]{$_\text{#1}$}
\newcommand{\rt}[1]{\begin{rotate}{30}#1\end{rotate}}



==> PEOPLES 2020 - Emotion in small datasets/figs/survey.tex <==
\begin{figure}[t]
    \begin{minipage}{.5\textwidth}
    \centering
    \includegraphics[width=.95\textwidth]{figs/when_equally_good.png}
    %\caption{\label{fig:survey1} Responses to survey question 1.}
    \end{minipage}
    %
    \begin{minipage}{.5\textwidth}
    \centering
    \includegraphics[width=.95\textwidth]{figs/when_dl_better.png}
    %\caption{\label{fig:survey2} Responses to survey question 2.}
    \end{minipage}
    \caption{\label{fig:survey}Responses to survey questions 1 (left) and 2 (right).}
\end{figure}


==> PEOPLES 2020 - Emotion in small datasets/figs/training_size.tex <==

\begin{figure}[t]
    \centering
    %\vspace*{-5pt}
    \includegraphics[width=.43\textwidth]{figs/fig_training_size.pdf}
    %\vspace*{-10pt}
    \caption{Comparison of model performance vs. training size on the SE07 dataset in Pearson's \textit{r}.}
    %\vspace*{-10pt}
    \label{fig:training_size}
\end{figure}

==> PEOPLES 2020 - Emotion in small datasets/tabs/cv_results.tex <==

\begin{table}[t]
    \centering
    \small
\vspace*{30pt}
\begin{tabular}{lccccc}                  
{} &  \rt{\textbf{SE07}} &  \rt{\textbf{WASSA}} &  \rt{\textbf{ANPST}} &   \rt{\textbf{MAS}} &  \rt{\textbf{Mean}} \\               
\midrule
Ridge\textsub{ngram} &     .53 &   .67 &   .32 &  .16 &  .42 \\                 
Ridge\textsub{BV}    &     .62 &   .64 &   .52 &  .62 &  .60 \\ 
CNN-LSTM &     .66 &   .69 &   .50 &  .63 &  .62 \\
CNN     &     \textbf{.67} &   .70 &   .47 &  .61 &  .62 \\
FFN     &     .67 &   .69 &   .50 &  .65 &  .63 \\
LSTM    &     .65 &   .73 &   .52 &  .65 &  .64 \\                   
GRU     &     .67 &   \textbf{.73} &   \textbf{.54} &  \textbf{.66} &  \textbf{.65} \\          
\midrule
\end{tabular}
%\vspace*{-3pt}
\caption{Comparative results of the $10{\times}10$-cross-validation in Pearson's $r$; averaged over all variables of the respective annotation format.}%; sorted by average over all data sets (`Mean').}
\label{tab:cv_results}
%\vspace*{-6pt}
\end{table}


==> PEOPLES 2020 - Emotion in small datasets/tabs/data.tex <==
\begin{table*}[t!]
    \centering
    \small
    \begin{tabular}{llrlrrlr}
    \toprule
        {\bf Corpus} & {\bf Language} & {\bf Size} & {\bf Annotation} & {\bf Emb. Alg.} & \textbf{Dims.} & {\bf Emb. Data} &  {\bf Emb. Data Size}\\
        \midrule
        SE07 & English & 1000 & BE6 $[1, 100]$ & word2vec & 300 & Google News  & 100B tokens\\
        %ANET & English & 120  & VAD $[1, 9]$&  FastText & Common Crawl & 600B \\
        WASSA & English & $\leq 2252$& BE4 $[0, 1]$ & word2vec & 400 & Twitter & 400M tweets \\
        ANPST & Polish & 718& VAD $[1, 9]$ & FastText & 300 & Wikipedia & 4B tokens\\
        MAS & Portuguese & 192 &  VAD $[1, 9]$ + BE5 $[1,5]$ & FastText & 300& Wikipedia  & 4B tokens \\
        \bottomrule
    \end{tabular}
    %\vspace*{-6pt}
    \caption{Annotated corpora and embedding models used for experiments; with language, number of instances, annotation format, embedding algorithm, embedding dimensions, and dataset (size) embeddings were trained on.}
    \label{tab:data}
    %\vspace{-6pt}
\end{table*}


==> PEOPLES 2020 - Emotion in small datasets/tabs/embedding_strategies.tex <==
\begin{table}[t]
\small
\center
% \begin{tabular}{lcccc}
% \toprule
% {} &  \bf Random &  \bf Learned & \bf Frozen & \bf Tuned \\
% \midrule
% FFN     &    .05 &     .24 &    \bf .63 &   .59 \\
% CNN     &    .15 &     .23 &    \bf .62 &   .55 \\
% GRU     &    .25 &     .38 &    \bf .65 &   .59 \\
% LSTM    &    .21 &     .26 &    \bf .64 &   .59 \\
% CNN-LSTM\hspace*{-.3cm}\vspace{.1cm} &    .20 &     .30 &   \bf .62 &   .57 \\
% \textbf{Mean}    &    .17 &     .28 &    \bf .63 &   .58 \\
% \bottomrule
% %\midrule
% \end{tabular}
\vspace*{.8cm}
\begin{tabular}{lccccccc}
{} &   \textbf{\rt{FFN}} &   \textbf{\rt{CNN}} &   \textbf{\rt{GRU}}&  \textbf{\rt{LSTM}} &  \textbf{\rt{CNN-LSTM}} &  \textbf{\rt{Mean}} \\
\midrule
\textbf{Learned} &  .24 &  .23 &  .38 &  .26 &     .30 &  .28 \\
\textbf{Tuned}   &  .59 &  .55 &  .59 &  .59 &     .57 &  .58 \\
\textbf{Frozen}  &  \textbf{.63} &  \textbf{.62} &  \textbf{.65} &  \textbf{.64} &     \textbf{.62} &  \textbf{.63} \\
\midrule
\end{tabular}
\vspace*{-6pt}
\caption{\label{tab:strategies}
Comparison of embedding training strategies (average Pearson's $r$ over all datasets).%; best result per row in bold).
}%\vspace*{-10pt}
\end{table}


==> PEOPLES 2020 - Emotion in small datasets/tabs/models.tex <==
\begin{table}
    \centering
    \small
    \begin{tabular}{p{1.7cm}p{4.9cm}}
    \toprule
    {\bf Model} &  {\bf Description}\\
    \midrule
     Ridge\textsub{ngram} & $n$-gram features with $n\in\{1,2,3\}$; feature normalization; automatically chosen regularization coefficient from $\{10^{-4}, 10^{-3}, .., 10^4\}$\\
     \midrule
     Ridge\textsub{BV}& \textit{bag of vectors}-features; regularization coefficient chosen as in `Ridge\textsub{ngram}'\\
    \midrule
     FFN    & \textit{bag of vectors}-features; two dense layers (256 and 128 units)\\
     \midrule
     CNN    & one conv. layer (filter size 3, 128 channels), max-pooling layer with .5 dropout; dense layer (128 units) \\
     \midrule
     GRU    & recurrent layer (128 units, uni-directional); last timestep receives .5 vertical dropout and is fed into a dense layer (128 units)\\
     \midrule
     LSTM   & identical to `GRU'\\
     \midrule
     CNN-LSTM & conv. layer as in `CNN'; max-pooling layer (pool size 2, stride size 1) with .5 dropout; LSTM identical to `GRU'\\
    \bottomrule
    \end{tabular}
    %\vspace*{0}
    \caption{Model-specific design choices.}
    %\vspace*{-12pt}
    \label{tab:models}
\end{table}

==> PEOPLES 2020 - Emotion in small datasets/tabs/semeval.tex <==
\begin{table}[b!]
    \centering
    \small
\vspace{10pt}
\begin{tabular}{lccccccc}
{} &  \textbf{\rt{Joy}} &  \textbf{\rt{Anger}} &  \textbf{\rt{Sadness}} &  \textbf{\rt{Fear}} &  \textbf{\rt{Disgust}} &  \textbf{\rt{Surprise}} &   \textbf{\rt{Mean}}   \\
\midrule
{\sc Winner}                         &  .23 &    .32 &      .41 &   .45 &      .13 &       .17 & .28 \\
IAA                          &  .60 &    .50 &      .68 &   .64 &      .45 &       .36 & .54  \\
{\sc Beck}              &  .59 &    .65 &      .70 &   .74 &      .54 &       .47 & .62 \\
GRU                      &  {\bf.60} &    {\bf.70} &      {\bf.75} &  {\bf .77} &      {\bf.61} &  {\bf.53} & {\bf.66}  \\
\midrule
\end{tabular}
\caption{Comparison of previously reported results, human performance (IAA), and our proposed GRU model on the SE07 dataset in Pearson's $r$.}
\label{tab:semeval}
\end{table}

==> PEOPLES 2020 - Emotion in small datasets/tabs/wassa.tex <==
\begin{table}[b!]
    \centering
    \small
\vspace{30pt}
\begin{tabular}{p{.5cm}lccccc}
\textbf{\rt{Official Rank}} & \textbf{\rt{Team/System}} & \textbf{ \rt{Joy}} &  \textbf{\rt{Anger}} &  \textbf{\rt{Sadness}} &  \textbf{\rt{Fear}} & \textbf{\rt{Mean}}   \\
\midrule
1 & Prayas & .762 & .765 & .732 & .732 & .747\\
2 & IMS & .726 & .767 & .690 & .705 & .722 \\
3 & SeeNet & .698 & .745 & .715 & .676 & .708 \\
-- & \textbf{Our Work} & .658 & .668 & .724 & .717 & .692\\
4 & UWaterloo & .699 & .703 & .693 & .643 & .685\\
\midrule
\end{tabular}
\caption{Comparison against official WASSA 2017 shared task results (in Pearson's $r$).}
\label{tab:wassa}
\end{table}

